Contrastive Losses Are Natural Criteria for Unsupervised Video Summarization

Video summarization aims to select the most informative subset of frames in a video to facilitate efficient video browsing. Unsupervised methods usually rely on heuristic training objectives such as diversity and representativeness. However, such methods need to bootstrap the online-generated summaries to compute the objectives for importance score regression. We consider such a pipeline inefficient and seek to directly quantify the frame-level importance with the help of contrastive losses in the representation learning literature. Leveraging the contrastive losses, we propose three metrics featuring a desirable key frame: local dissimilarity, global consistency, and uniqueness. With features pre-trained on the image classification task, the metrics can already yield high-quality importance scores, demonstrating competitive or better performance than past heavily-trained methods. We show that by refining the pre-trained features with a lightweight contrastively learned projection module, the frame-level importance scores can be further improved, and the model can also leverage a large number of random videos and generalize to test videos with decent performance. Code available at https://github.com/pangzss/pytorch-CTVSUM.

==> notes.tex <==
Though unq works well for TVsum videos, it hardly brings any benefits for the summe videos. Thus the good performance of the uniquness filter for TVSum may simply stem from the fact that the background frames in TVSum are not challenging enough and can be easily detected by the uniqueness filter trained using few videos. Therefore, we suppose that the uniqueness filter needs to be trained on more videos in order to filter out more challenging background frames such that it can generalize to a wider range of videos. 

unif not working for summe: however, we believe that this is a deficiency of not only our method, but it should be a common concern for the current approaches that are leveraging reconstruction-based representativeness objectives and the future attempts that will consider using it. We advocate for efforts in exploring other possibilities to achieve representativeness and are interested in this meaningful future direction. 


During contrastive refinement, there are four situations:
1. a frame does not have a sufficient amount of positive samples such that pos contains semantically disparate samples. In this case, laln will be difficult to minimize and lunif is easily minimized.

2. a frame has a sufficient amount of positive samples, but not related to most of the frames in the video, the laln will be easily minimized and lunif can also be easily minimized

3. a frame has 
